Sub-galactic scaling relations with T$_{\rm e}$-based metallicity of low metallicity regions in galaxies: metal-poor gas inflow may have important effects?

The scaling relationship is a fundamental probe of the evolution of galaxies. Using the integral field spectroscopic data from the Mapping Nearby Galaxies at Apache Point Observatory survey, we select 1698 spaxels with significant detection of the auroral emission line \oiii$\lambda$4363 from 52 galaxies to investigate the scaling relationships at the low-metallicity end. We find that our sample's star formation rate is higher and its metallicity is lower in the scaling relationship than the star-forming sequence after removing the contribution of the Fundamental Metallicity Relation.We also find that the stellar ages of our sample are younger ($<$ 1 Gyr) and the stellar metallicities are also lower. Morphological parameters from Deep Learning catalog indicate that our galaxies are more likely to be merger. These results suggest that their low metallicity regions may be related to interaction, the inflow of metal-poor gas may dilute the interstellar medium and form new metal-poor stars in these galaxies during interaction.

==> backup.tex <==
\section{Others} \label{sec:others}

\subsection{Selection Effect}
We have noticed that in order to ensure low error of metal abudance we only selected [OIII]$\lambda$4363 emission lines with high signal-to-noise, but [OIII]$\lambda$4363 emission line is indeed a very weak line, which can’t be detected in most MaNGA spaxels. This will cause a certain selection effect. Only spaxels close enough to us, high enough in brightness, and low enough in metal abundance can be selected by us. And those that meet the $\Sigma_*-$Z relationship are likely to be excluded because of their dimness and small number.

In order to estimate the impact of the selection effect, we have conducted a series of simulated selection processes. We use the star forming spaxels sample of \cite{2018ApJ...868...89G}. We first take the converted O3N2 metal abundance as the true metal abundance, and then use the electronic temperature method \citep{2006A&A...448..955I} to inversely resolve the flux of [OIII]$\lambda$4363 emission line. We regard the noise of Hbeta as the noise of [OIII]$\lambda$4363, so that we get the estimated value of the signal-to-noise ratio of each spaxel. This sample is bigger and more complete than mine, which is more suitable for evaluating the selection effect.

In order to verify the accuracy of our estimated flux, we compare our estimated flux with real and reliable existed observation data. There are 883 such spaxels in their sample. Figure \ref{fig:obs_vs_est_4363} is the comparison between our back-estimated results and actual observations. It can be seen that the estimated and observed values are basically the same. The point of inconsistency in the upper left corner is caused by too low ionization parameters. If the ionization parameter is too low, the O3N2 metalicity will be too high, and the estimated value of [OIII]$\lambda$4363 flux will be too low.

\begin{figure}[ht!]
	\plotone{obs_vs_est_4363.pdf}
	\caption{The comparison between our estimated flux with real and reliable existed observation data  \label{fig:obs_vs_est_4363}}
\end{figure}

\begin{figure}[ht!]
	\includegraphics[width=1\textwidth]{select_effect_1.png}
	\caption{select effect 1.png  \label{fig:select_effect_1}}
\end{figure}

Figure \ref{fig:select_effect_1} shows the effect of different signal-to-noise ratio truncation on the $\Sigma_*$-$\Sigma_{\rm SFR}$ and $\Sigma_-*$Z of the selected samples. We can see that as the signal-to-noise ratio increases, the SFR of the selected samples continues to increase and the metal abundance continues to decrease. And they move to the lower left on the $\Sigma_*$-$\Sigma_{\rm SFR}$ relation, and move to the lower right on the $\Sigma_-*$Z relation. Figure \ref{fig:select_effect_result} shows the trend of the average metal abundance and mass surface density of the selected samples with the signal-to-noise ratio. We can see that the higher signal-to-noise ratio truncation will indeed result in a higher mass surface density and lower metal abundance in the selected samples. The signal-to-noise ratio increased from 0 to 10, and the average mass surface density increased from 7.3 to 7.6. The metal abundance decreased from 8.3 to 8.2. But it is not enough to shift to around 8, which is still not enough to produce the observed results.

\begin{figure}[ht!]
	\includegraphics[width=1\textwidth,trim=70 0 70 0,clip]{select_effect_result.pdf}
	\caption{select effect result.pdf  \label{fig:select_effect_result}}
\end{figure}

\subsection{Possible Reasons Why [OIII]$\lambda$4363 Selected Spaxels Deviates from The Normal Spaxels}
In previous studies, extreme metal-poor galaxies selected by [OIII]$\lambda$4363 methods reported have similar results where M$-$Z relation of extreme metal-poor galaxies is systematically lower than the main sequence. The outlier can be explained by some reasons such as selection effect, gravitational interactions, etc. \citep{2010MNRAS.406.1238E, 2015ApJ...802...82F, 2020ApJ...891..181M}.  In this work, we will discuss the intrinsic dispersion between different metallicity calculation method, the selection effect and an actual existed population.
\subsubsection{Evidence of Accretion: Morphology} \label{subsubsec:img}
Most of our samples are strongly asymmetric galaxies. \cite{2019ApJ...872..144H} has discussed it.
\subsection{The Star Formation History}
After the discussion in the previous section, we have determined that the samples we selected based on the [OIII]4363 auroral line are indeed the ALM region below the main sequence of star formation in the $\Sigma_*-$Z plane. In order to better understand the causes of these ALM regions, we can analyze their star formation history.

The fitting program pPXF we use can give the weight of each template, so that we can get a non-parametric star formation history of each spectrum. Because the signal-to-noise ratio of the IFU spectrum is low, and there is the influence of the point spread function(PSF). We stack all the spectra of the sample spaxels of each galaxy and refitted it again to ensure a higher signal-to-noise ratio and reduce the effect of PSF. We select 40 galaxies whose signal-to-noise ratios of stacked spectra are greater than 10 from 43 sample galaxies, and results are shown in Figure \ref{fig:sfh_mat}. We find that they all have two stellar components, one old population (> 5 Gyr) and one young population (< 100 Myr). This is consistent with the ALM lifetimes estimated by \cite{2019ApJ...872..144H}. For the fitted stellar metal abundance, we find that the metal abundance of the new stellar composition is lower than that of the old. This could mean that the interstellar medium (ISM) used to form stars is diluted with metal-poor gas.


\begin{figure}[ht!]
	\includegraphics[width=1\textwidth,trim=90 0 200 0,clip]{sfh_mat.pdf}
	\caption{The stellar component of the stacked spectra of 40 galaxies in our sample. The colored value on the age-metallicity grid point is the quantity of galaxies whose stacked spectra can derive corresponding stellar component. Each gray line is the ratio of the mass surface density of stellar at the corresponding age in the stacked area to the total mass surface density of this area. Black line is the average value of these 40 gray lines. \label{fig:sfh_mat}}
\end{figure}

Then, in order to study what component caused the abnormally high mass surface density. Here we divide our samples into “abnormal” samples ($\log{\rm \Sigma_*}>$8) and “normal” samples ($\log{\rm \Sigma_*}$<8). Then draw the curves of their stars formation history. We find that the difference in the mass surface density between the normal and abnormal samples is mainly caused by the old star population (Figure 11 shows an example), while the young star population has almost no difference in the mass surface density. In theory, galaxies with such high mass surface density should have higher metal abundance, but they do not. It means that their enriched metal has more outflow, or that extra metal-poor gas has flowed into the galaxy, causing dilution. The former is unlikely because of the higher total mass and mass surface density. Combined with the lower metal abundance of newly formed stars, we believe that the newly flowing gas into the galaxy caused its metal to be diluted and triggered the formation of new stars.

\subsection{Systematic Error with Strong Line Method} \label{subsec:systematic_error}

In Section \ref{subsec:m_sfr_z_relation}, we have compared the $\Sigma_*-$Z relation between our sample and the star forming main sequence in \cite{2018ApJ...868...89G}. However, due to the lack of [OIII]$\lambda$4363 observation, we can only use strong line ratios to estimate metallicities of normal star forming spaxels. There are systematic errors between different methods, so it is not suitable for direct comparison. It is very necessary for us to discuss this issue.

For normal star forming samples of \cite{2018ApJ...868...89G}, to ensure consistency with $T_{\rm e}$ method, we have already transformed the metallicity by Eq. \ref{eq:o3n2_transform}. For our [OIII] selected samples, their metallicities are poorer, and other parameters could be more extreme than those with common metallticity. The lower left panel of Figure \ref{fig:overall_properties} shows that our sample has extremely high ionization parameters, which may cause inconsistencies between different methods. For IFS observations like MaNGA, it can be important to consider the influence of the ionization structure of HII regions. This behavior can be seen clearly in Figure 13 of \cite{2011MNRAS.411.2076L}.

In Figure \ref{fig:te_cmp_o3n2}, we have compared our samples with the calibration of \cite{2013A&A...559A.114M}(M13) and \cite{2004MNRAS.348L..59P}(PP04), and evaluated the influence of ionization parameter. We find that our samples distributed in O3N2$-$Z plane are consistent with the M13, and the systematic error of the 2 method is only 0.03 dex, while the typical error of $T_{\rm e}$-based metallicity is 0.13 dex. This means that the systematic error caused by different metallicity calculation methods is much smaller than the measurement error. Therefore, we can think that our results are able to be directly compared with the M13 method. For ionization parameter, the result is the same as \cite{2011MNRAS.411.2076L}, showing that higher ionization parameter may result in an underestimation of metal abundance by O3N2 method.


\begin{figure}[ht!]
	\includegraphics[width=1\textwidth,trim=50 0 50 30,clip]{te_cmp_o3n2.pdf}
	\caption{Left panel: Metal abundance versus the O3N2 index for $T_{\rm e}$-based abundances. The black solid line is the M13 calibration. The gray region around the black solid line is encompass 1$\sigma$ ($\pm$0.18 dex) of all measurements in M13. The black dashed line is the PP04 calibration. Green dots are the new CALIFA-$T_{\rm e}$ data in M13. Right panel: Relation between the ionization degree, given by the reddening-corrected [OIII]$\lambda$5007/[OII]$\lambda$3727 ratio, and the residuals of metal abundance between $T_{\rm e}$ method and O3N2 calibration ($\Delta$[12+log(O/H)]=[12+log(O/H)$_{\rm Te}$]-[12+log(O/H)$_{\rm O3N2,M13}$]). The blue solid line is the average value of our samples. The black dotted lines on the upper and lower sides of the 0 horizontal dashed line represent the typical error of $T_{\rm e}$-based abundances. The blue dots in both panels are our samples. \label{fig:te_cmp_o3n2}}
\end{figure}


\subsection{Influence of Nebular Free-bound Continuum Emission}
We have found that our all samples are young and metal-poor. This makes it critical for us to consider the effects of free-bound radiation of nebular\citep{2013ARA&A..51..393C}. We make use of STARBURST99 which  \citep{1999ApJS..123....3L} to evaluate the effect of free-bound continuum emission on the fit. STARBURST99 is a comprehensive set of model predictions for spectrophotometric and related properties of galaxies with active star formation. Its metallicity coverage is between Z=0.040 and 0.001 and the age coverage is $10^6-10^9$ yr.

\subsection{Rotation curve}
To find evidence of new gas inflows, we analyzed the kinematics of stars and gas in our galaxy. We directly use the MaNGA DAP data here. It can provide the ionizing gas emission line (H$\alpha$, etc.) and the star's radial velocity. We obtain the rotation curve of the galaxy by the following method.


\begin{enumerate}
	\item Obtain the line-of-sight velocity Map of the ionized gas H$\alpha$ from the DAP, take the absolute value and then average. Find the spaxels whose absolute value of velocity is greater than the average.
	\item Then use a straight line with the center of the galaxy as the origin to perform a least squares fit on these points. The fitted straight line is set as the plane of rotation of the gas.
	\item Check the fitted line manually, and reset the slope if the fitted line is obviously inconsistent with the rotation plane.
	\item Along the determined rotation plane, calculate the distance to the center from left to right (with $b/a$ correction), and read the gas and star velocities from the DAP to obtain the rotation curve.
\end{enumerate}

We have drawn the rotation curves of 10 galaxies with relatively regular shapes, and found that some of them such as 8313-1901 and 8727-3702 have a phenomenon in which gas and stars rotate in different directions. Their velocity map and r rotation curves are shown in Figure \ref{fig:8313-1901_rot_curve}. This is generally evidence of gas inflow (相关文献待查).

\begin{figure}[ht!]
	\includegraphics[width=1\textwidth]{8313-1901_rot_curve.pdf}
	\includegraphics[width=1\textwidth]{8727-3702_rot_curve.pdf}
	\caption{8313-1901 and 8727-3702  \label{fig:8313-1901_rot_curve}}
\end{figure}
